A Digital Language Coherence Marker for Monitoring Dementia

The use of spontaneous language to derive appropriate digital markers has become an emergent, promising and non-intrusive method to diagnose and monitor dementia. Here we propose methods to capture language coherence as a cost-effective, human-interpretable digital marker for monitoring cognitive changes in people with dementia. We introduce a novel task to learn the temporal logical consistency of utterances in short transcribed narratives and investigate a range of neural approaches. We compare such language coherence patterns between people with dementia and healthy controls and conduct a longitudinal evaluation against three clinical bio-markers to investigate the reliability of our proposed digital coherence marker. The coherence marker shows a significant difference between people with mild cognitive impairment, those with Alzheimer's Disease and healthy controls. Moreover our analysis shows high association between the coherence marker and the clinical bio-markers as well as generalisability potential to other related conditions.

==> literature.tex <==
\section{Related Work}

\paragraph{Computational Approaches for dementia diagnosis:}
Early work for using NLP for dementia detection analysed aspects of language such as lexical, grammatical, and semantic features \cite{ahmed2013connected,orimaye2017predicting,kave2018severity}, showing that people with dementia produced less lexical and semantic context and lower syntactic complexity compared to healthy controls. Lack of fluency through the study of paralinguistic features has also been shown to be indicative of people with dementia \cite{lopez2013selection}. The semantics and pragmatics of their language appear affected throughout the entire span of the disease, more so than syntax \cite{bayles1982potential}. In particular, people with dementia talk more slowly with longer pauses \cite{gayraud2011syntactic,lopez2013selection,pistono2019happens}. \\
%\vspace{-0.2cm}
Recent work investigated manually engineered acoustic features to recognize AD from spontaneous speech \cite{luz2020alzheimer,luz2021detecting} while other work exploited non-linguistic features to distinguish people with AD from healthy controls \cite{nasreen2021detecting}. %Another direction in this field exploited NLP techniques on the linguistic modality, such as LSTM and CNN 
Neural models such as LSTM and CNN\cite{karlekar2018detecting} or pre-trained language models \cite{yuan2020disfluencies}, have been used to analyze disfluency characteristics, such as filled pauses. Researchers have used neural approaches to extract either acoustic features  \cite{pan2020acoustic,pan2021using} or linguistic information \cite{zhu2021wavbert} directly from the speech signal for dementia detection. Existing work has focused on distinguishing people with dementia from healthy controls without considering language changes over time. Here we investigate changes in language coherence from a longitudinal aspect and how such changes relate to changes in cognitive status.\\
%\vspace{-0.4cm}
\noindent \textbf{Coherence Models for Text:}
Most work in this space focusses on modelling coherence within documents. Early work focused on feature engineering to realize some of the intuitions of Centering Theory \cite{grosz1995centering}. In particular, it exploited features based on local entities and lexical transitions \cite{lapata2005automatic,barzilay2008modeling,elsner2011extending,guinaudeau2013graph} as well as more global concerns regarding topic transitions \cite{elsner2007unified}. Driven by the success of deep neural networks, many neural models were proposed in the past few years. \citet{cui2017text} proposed a distributional sentence model based on convolutional neural networks to capture document coherence. \citet{xu2019cross} introduced a neural discriminative model to compute the local coherence score of documents by estimating a coherence probability for pairs of sentences. \citet{feng2021towards} trained a BERT-based model of text coherence to estimate the probability that a given sentence will come next in a story. Recently, the text coherence task has been approached in a zero-shot setting using generative and bi-directional transformers \cite{laban2021can}. Their results showed that large architectures achieved high performance out-of-the-box. Here we investigate a variety of SOTA coherence models for modelling coherence in sequences of sentences in order to learn language coherence from healthy controls in the Pitt corpus~\cite{becker1994natural}.

